Observations and Modelling of the Pre-Flare Period of the 29 March 2014 X1 Flare

On the 29 March 2014 NOAA active region (AR) 12017 produced an X1 flare which was simultaneously observed by an unprecedented number of observatories. We have investigated the pre-flare period of this flare from 14:00 UT until 19:00 UT using joint observations made by the Interface Region Imaging Spectrometer (IRIS) and the Hinode Extreme Ultraviolet Imaging Spectrometer (EIS). Spectral lines providing coverage of the solar atmosphere from chromosphere to the corona were analysed to investigate pre-flare activity within the AR. The results of the investigation have revealed evidence of strongly blue-shifted plasma flows, with velocities up to 200 km/s, being observed 40 minutes prior to flaring. These flows are located along the filament present in the active region and are both spatially discrete and transient. In order to constrain the possible explanations for this activity, we undertake non-potential magnetic field modelling of the active region. This modelling indicates the existence of a weakly twisted flux rope along the polarity inversion line in the region where a filament and the strong pre-flare flows are observed. We then discuss how these observations relate to the current models of flare triggering. We conclude that the most likely drivers of the observed activity are internal reconnection in the flux rope, early onset of the flare reconnection, or tether cutting reconnection along the filament.

==> SOLA_example_labels.tex <==
This file contains the command names and the labels used in
the associated .tex file.    It is useful to have present file open
as the same time of the .tex file to copy/paste definitions.
When a new definition is added, it is important to keep this file
updated. 

   % Copy/paste of the definitions used in the .tex
\newcommand{\BibTeX}{\textsc{Bib}\TeX}
\newcommand{\etal}{{\it et al.}}

% Definitions for equations
\newcommand{\deriv}[2]{\frac{{\mathrm d} #1}{{\mathrm d} #2}}
\newcommand{\rmd}{ {\ \mathrm d} }
\renewcommand{\vec}[1]{ {\mathbf #1} }
\newcommand{\uvec}[1]{ \hat{\mathbf #1} }
\newcommand{\pder}[2]{ \f{\partial #1}{\partial #2} }
\newcommand{\grad}{ {\bf \nabla } }
\newcommand{\curl}{ {\bf \nabla} \times}
\newcommand{\vol}{ {\mathcal V} }
\newcommand{\bndry}{ {\mathcal S} }
\newcommand{\dv}{~{\mathrm d}^3 x}
\newcommand{\da}{~{\mathrm d}^2 x}
\newcommand{\dl}{~{\mathrm d} l}
\newcommand{\dt}{~{\mathrm d}t}
\newcommand{\intv}{\int_{\vol}^{}}
\newcommand{\inta}{\int_{\bndry}^{}}
\newcommand{\avec}{ \vec A}
\newcommand{\ap}{ \vec A_p}
\newcommand{\bb}{ \vec B}
\newcommand{\jj}{ \vec j}
\newcommand{\rr}{ \vec r}
\newcommand{\xx}{ \vec x}

% Definitions for the journal names
\newcommand{\adv}{    {\it Adv. Space Res.}} 
\newcommand{\annG}{   {\it Ann. Geophys.}} 
\newcommand{\aap}{    {\it Astron. Astrophys.}}
\newcommand{\aaps}{   {\it Astron. Astrophys. Suppl.}}
\newcommand{\aapr}{   {\it Astron. Astrophys. Rev.}}
\newcommand{\ag}{     {\it Ann. Geophys.}}
\newcommand{\aj}{     {\it Astron. J.}} 
\newcommand{\apj}{    {\it Astrophys. J.}}
\newcommand{\apjl}{   {\it Astrophys. J. Lett.}}
\newcommand{\apss}{   {\it Astrophys. Space Sci.}} 
\newcommand{\cjaa}{   {\it Chin. J. Astron. Astrophys.}} 
\newcommand{\gafd}{   {\it Geophys. Astrophys. Fluid Dyn.}}
\newcommand{\grl}{    {\it Geophys. Res. Lett.}}
\newcommand{\ijga}{   {\it Int. J. Geomagn. Aeron.}}
\newcommand{\jastp}{  {\it J. Atmos. Solar-Terr. Phys.}} 
\newcommand{\jgr}{    {\it J. Geophys. Res.}}
\newcommand{\mnras}{  {\it Mon. Not. Roy. Astron. Soc.}}
\newcommand{\nat}{    {\it Nature}}
\newcommand{\pasp}{   {\it Pub. Astron. Soc. Pac.}}
\newcommand{\pasj}{   {\it Pub. Astron. Soc. Japan}}
\newcommand{\pre}{    {\it Phys. Rev. E}}
\newcommand{\solphys}{{\it Solar Phys.}}
\newcommand{\sovast}{ {\it Soviet  Astron.}} 
\newcommand{\ssr}{    {\it Space Sci. Rev.}} 

%%%%%%%%%%%%%%%% Roadmap of the paper with all the labels %%%%%%%%%%%%%%%%%%%%%%%%
%%%% (with the exception of citations since author-year is easy to remember) %%%%%
1 Section~\ref{S-Introduction}
2 Section~\ref{S-general}
  Section~\ref{S-text}
  Section~\ref{S-labels}
3 Section~\ref{S-features}
  Section~\ref{S-equations}
   Section~\ref{S-simple-equations}
     Equation~(\ref{Eq-H-def})
   Section~\ref{S-array-equations}
     Equation~(\ref{Eq-A-B})
     Equation~(\ref{Eq-H-B})
     Equation~(\ref{Eq-H-N})
   Section~\ref{S-long-equations}
     Equation~(\ref{Eq-dH-Phi})  
  Section~\ref{S-figures}
  Section~\ref{S-tables}
  Section~\ref{S-references}
  Section~\ref{S-BibTeX}
  Section~\ref{S-Miscellaneous}
4 Section~\ref{S-Conclusion}

A Appendix~\ref{S-appendix}
 
 1 Figure~\ref{F-simple}
 2 Figure~\ref{F-4panels}
 3 Figure~\ref{F-rotate-cut}
 4 Figure~\ref{F-appendix}

 1 Table~\ref{T-simple}
 2 Table~\ref{T-complex}
 3 Table~\ref{T-appendix}

%%%%%%%%%%%%%%%%%%%% Results for the citation commands %%%%%%%%%%%%%%%%%%%%%%%%  
\cite{Kusano04}          : (Kusano \etal, 2004)
\cite{Kusano04,Berger03} : (Kusano \etal, 2004; Berger, 2003)
\inlinecite{Brown99}     : Brown, Canfield, and Pevtsov (1999)
\opencite{Brown99}       : Brown, Canfield, and Pevtsov, 1999
\citeauthor{Brown99}     : Brown, Canfield, and Pevtsov
\shortcite{Brown99}      : (1999)
\citeyear{Brown99}       : 1999
(\opencite{Berger84}, \citeyear{Berger03}) 
                         : (\opencite{Berger84}, \citeyear{Berger03})


